Simple Mechanisms for Subadditive Buyers via Duality

We provide simple and approximately revenue-optimal mechanisms in the multi-item multi-bidder settings. We unify and improve all previous results, as well as generalize the results to broader cases. In particular, we prove that the better of the following two simple, deterministic and Dominant Strategy Incentive Compatible mechanisms, a sequential posted price mechanism or an anonymous sequential posted price mechanism with entry fee, achieves a constant fraction of the optimal revenue among all randomized, Bayesian Incentive Compatible mechanisms, when buyers' valuations are XOS over independent items. If the buyers' valuations are subadditive over independent items, the approximation factor degrades to $O(\log m)$, where $m$ is the number of items. We obtain our results by first extending the Cai-Devanur-Weinberg duality framework to derive an effective benchmark of the optimal revenue for subadditive bidders, and then analyzing this upper bound with new techniques.

==> appx_duality.tex <==
%\section{Missing Details of Section~\ref{sec:duality}}\label{sec:appx_duality}



==> computation.tex <==

\section{Efficiently Finding the Mechanism for Identical Bidders}
In this section, we are going to prove that such a mechanism which approximately obtains the optimal revenue can be computed in polynomial time when bidders are identical. To say \textbf{identical}, we mean all bidders share same private information set $\tilde{T}$ and distribution $\tilde{D}$ on this support. Besides, given a same private information, all bidders have the same item valuation, i.e., for any $t\in \tilde{T}$ and $S\subseteq [m]$, $v_i(t,S)=v_j(t,S)$ holds for all $i,j\in [n]$.

When bidders are identical, it's reasonable to only consider symmetric mechanisms. In a symmetric mechanism, the ex-ante probability to win an item $j$ is the same for all bidder $i$, and thus no more than $\frac{1}{n}$ due to no overallocation. The following lemma formally proves these observations.

\begin{lemma}\label{lem:comp:symmetric}
If bidders are identical, then for any BIC mechanism $M$, there exists a symmetric BIC mechanism $M'$ that satisfies
\begin{itemize}
\item $\rev(M,v,D)=\rev(M',v,D)$
\item $\forall i\in [n], \sum_{t_i\in T_i}f_i(t_i)\cdot \pi_{ij}'(t_i)\leq \frac{1}{n}$
\end{itemize}
where $\pi_{ij}'(t_i)=\sum_{S:j\in S}\sigma_{iS}'(t_i)$ and $\sigma_{iS}'(t_i)$ is the probability of buyer i receiving exactly bundle S when her reported type is $t_i$ in mechanism $M'$.
\end{lemma}
\begin{proof}
Define mechanism $M'$ as follows: after receiving type profile $t=\langle t_i\rangle_{i=1}^n$, draw a random permutation $\rho$ of size $n$. Then follow mechanism $M$ treating bidder $i$ as $\rho(i)$ for all $i$. Formally, we denote by $M_i(t)$, $h_i(t)$ the (probably random) received item set and charged price to bidder $i$ by mechanism $M$ when type profile is $t$, and $M_i'(t)$, $h_i'(t)$ the same meaning for mechanism $M'$. After the permutation $\rho$ is drawn, define type profile $t^{(\rho)}=\langle t_{\rho(i)}\rangle_{i=1}^n$. The allocation rule and price for mechanism $M'$ is then defined as: $M_i'(t)=M_{\rho(i)}(t^{(\rho)})$, $h_i'(t)=h_{\rho(i)}(t^{(\rho)})$. Since bidders are identical, with the random permutation, $M'$ will treat all bidders as a same role, and thus the ex-ante probability getting an item $j$ is the same for all bidders. Clearly $\sum_i\sum_{t_i\in T_i}f_i(t_i)\cdot \pi_{ij}'(t_i)\leq 1$, thus each ex-ante probability $\sum_{t_i\in T_i}f_i(t_i)\cdot \pi_{ij}'(t_i)\leq \frac{1}{n}$.

To prove that $M'$ has the same expected revenue as $M$, it's enough to show $\sum_t f(t)\cdot \sum_i h_i(t)=\sum_t f(t)\cdot \sum_i h_{\rho(i)}(t^{(\rho)})$. Notice for all $t\in T$, $f(t)=f(t^{(\rho)})$ as all bidders' types are independent, we have
\begin{equation}
\sum_t f(t)\cdot \sum_i h_{\rho(i)}(t^{(\rho)})=\sum_t f(t^{(\rho)})\cdot \sum_i h_i(t^{(\rho)})=\sum_t f(t)\cdot \sum_i h_i(t)
\end{equation}

%Now we show $M'$ is a BIC mechanism.

\end{proof}

Now without loss of generality, we can assume $M$ is a symmetric mechanism. For every $i\in [n], j\in [m]$, select $\beta_{ij}$ such that $\Pr_{t_{ij}}\left[V_i(t_{ij})\geq \beta_{ij}\right]=\frac{b}{n}$. With Lemma~\ref{lem:comp:symmetric}, it's easy to check that $\beta$ satisfies the two conditions in Lemma~\ref{lem:requirement for beta} and thus Theorem~\ref{thm:multi} works. We have to note here that in a discrete distribution $D_{ij}$, there might not exist such a $\beta_{ij}$. Thus we have to assume that $\forall i,j, \exists \beta_{ij}$ such that $\Pr_{t_{ij}}\left[V_i(t_{ij})\geq \beta_{ij}\right]=\frac{b}{n}$, so that it's able to get the exact $\beta_{ij}$. $\beta_{ij}$ is sensitive to the proof and the mechanism used in the proof, and thus it's necessary to use the exact value.

Consider this specific $\beta$ for proofs in Section~\ref{sec:multi}. Now we'll show all the posted price and entry fee for the mechanisms that we use in the proof can be computed in polynomial time.

Given bidder $i$'s type $t_i$, it'll need exponential size to explicitly described $i$'s value $v_i(t_i,\cdot):2^{[m]}\to R^{*}$. Thus it's usually assumed that there exist the following oracles access to $v_i(\cdot,\cdot)$.

\begin{itemize}
\item Value oracle: Given type $t_i\in T_i$ and set $S$ as input, returns a non-negative real number that represents bidder's value $v_i(t_i,S)$.
\item XOS oracle(for XOS valuations): Given type $t_i\in T_i$ and set $S$ as input, returns prices $\{p_j\}_{j\in S}$ as the 1-supporting prices for $v_i(t_i,S)$.
\end{itemize}

We now state the main theorem for this section:
\begin{theorem}
Consider the case that bidders are identical, and have XOS valuations. Suppose $\forall i,j, \exists \beta_{ij}$ such that $\Pr_{t_{ij}}\left[V_i(t_{ij})\geq \beta_{ij}\right]=\frac{b}{n}$. Besides, we are given
\begin{itemize}
\item $\forall i,j$, the distribution for $v_i(t_{ij})$.
\item $\forall i\in [n]$, a value oracle for $v_i(\cdot,\cdot)$.
\item $\forall i\in [n]$, an XOS oracle for $v_i(\cdot,\cdot)$.
\item $\forall t\in T$, a black box algorithm $\mathcal{A}$ that maximizes the social welfare for the combinatorial auction with bidder's valuation $v_i'(t_i,\cdot)$.
\end{itemize}

Then with $O()$ type samples from $T$, with probability at least ---, we can compute a DSIC mechanism in $POLY(n,m,\sum_i\sum_j |T_{ij}|, )$ time such that the revenue of this mechanism obtains at least $1/$ the optimal revenue.
\end{theorem}

\begin{proof}
Firstly for Lemma~\ref{lem:multi_single}, as showed in \cite{ChawlaHMS10, KleinbergW12}, the posted-price mechanism that used can be efficiently computed. We now consider the Sequential Posted Price Mechanism stated in Section~\ref{subsection:tail} and Section~\ref{subsection:core}.

The mechanism used in Corollary~\ref{cor:bound tail } is determined by the posted price $\xi_{ij}=\beta_{ij}+P_{ij}$. Having distribution $D_{ij}$, $\beta_{ij}$ and $P_{ij}$ can both be computed in $O(|T_{ij}|)$ time by brute force. Thus this mechanism can be computed in linear time.

Now consider the ``CORE" part. Recall that $\core(\beta)=\sum_i\sum_{t_i\in T_i}f_i(t_i)\cdot \sum_{S\subseteq[m]}\sigma_{iS}^{(\beta)}(t_i)\cdot v'_i(t_i,S)$, which can be described as the expected social welfare of $M^{(\beta)}$ in a new combinatorial auction. In this auction, when type profile $t\in T$, bidder $i$ has valuation $v_i'(t_i,\cdot)$. Let $M^{(\beta),*}$ be the optimal mechanism among above and $\sigma_{iS}^{(\beta),*}$, $Q_j^{*}$ be the corresponding definition. Then according to Lemma~\ref{lem:core and q_j}, $2\alpha\cdot\sum_{j\in [m]}Q_j^{*}\geq \core(\beta)$ holds for all BIC mechanism $M^{(\beta)}$. It implies that the mechanism with specific parameter $\beta$ and $\sigma_{iS}^{(\beta)}=\sigma_{iS}^{(\beta),*}$ can guarantee a constant factor of the optimal revenue.

The Sequential Posted Price Mechanism with Entry Fee stated in Section~\ref{subsection:core} use $Q_j^{*}$ as the posted price for item $j$. Recall that $Q_j^{*}=\frac{1}{2}\cdot \sum_i \sum_{t_i\in T_i}f_i(t_i)\cdot\sum_{S:j\in S}\sigma_{iS}^{(\beta),*}(t_i)\cdot \gamma_j^{S}(t_i)$. Even exactly calculating one $\sigma_{iS}^{(\beta),*}(t_i)$ requires running mechanism $M^{(\beta),*}$ under every type profile $t$, which takes exponential time. $Q_j^{*}$ can thus not be able to compute exactly in polynomial time.




%Then consider the Sequential Posted Price Mechanism without Entry Fee stated in Lemma~\ref{lem:beta_ij} and \ref{lem:tau_i}, which takes posted price as $\max\{\beta_{ij},Q_j+\tau_i\}$. 

Recall that $Q_j=\frac{1}{2}\cdot \sum_i \sum_{t_i\in T_i}f_i(t_i)\cdot\sum_{S:j\in S}\sigma_{iS}^{(\beta)}(t_i)\cdot \gamma_j^{S}(t_i)$. And even exactly calculating one $\sigma_{iS}^{(\beta)}(t_i)$ requires running mechanism $M$ under every type profile $t$, which takes exponential time. $Q_j$ can thus not be able to compute exactly in polynomial time. What we do is to generate enough samples of type profile $t\in T$, run $M$ with those samples, and calculate the empirical approximation for $Q_j$.







\end{proof}


Corollary~\ref{cor:bound tail }, Lemma~\ref{lem:beta_ij}, Lemma~\ref{lem:tau_i}, and Definition~\ref{def:entry fee}.






==> proof_concentration.tex <==
\section{Proof of Corollary~\ref{corollary:concentrate}}\label{sec:concentration_proof}



==> proof_valuation_relaxation_2.tex <==
\section{Proof of Lemma~\ref{lem:relaxed valuation}}
\begin{lemma}\label{lem:relaxed valuation stronger}
	In a $n$-player $m$-item combinatorial auction, for any absolute constant $\eta\in(0,1)$ and $\epsilon>0$, any two type profile distributions $D, D'$ on type profile set $T$ and $T'$ accordingly($T$ and $T'$ might be different), any two valuation functions $\{v_i(\cdot,\cdot)\}_{i\in[n]}$, $\{v_i'(\cdot,\cdot)\}_{i\in[n]}$,  assume for every $i$ there exists a coupling $\hat{D_i}$ for $D_i$ and $D_i'$ such that $\forall t_i\in T_i,t_i'\in T_i', \hat{D_i}(t_i,t_i')>0$, $v_i'(t_i',S)\geq v_i(t_i,S)$ holds for subset $S$. Here $\hat{D_i}(t_i,t_i')$ is the coupling probability. Then for any BIC mechanism $M$ for valuation functions $\{v_i(\cdot,\cdot)\}_{i\in[n]}$ with respect to $D$, there exists a BIC mechanism $M'$ for valuation functions $\{v_i'(\cdot,\cdot)\}_{i\in[n]}$ with respect to distribution $D'$, such that
	\begin{enumerate}
		\item $\sum_{t_i'\in T_i'}f_i'(t_i')\cdot\sum_{S: j\in S}\sigma'_{iS}(t_i')\leq \sum_{t_i\in T_i}f_i(t_i)\cdot\sum_{S: j\in S}\sigma_{iS}(t_i)$, for all $i$ and $j$,
		\item $\rev(M, v, D)\leq$\\
$~~~~\frac{1}{1-\eta}\cdot{\rev(M',v', D')}+\frac{1}{\eta}\cdot \sum_i\sum_{t_i'\in T_i'}\sum_{t_i\in T_i}\sum_{S\subseteq[m]}\hat{D_i}(t_i,t_i')\cdot\sigma'_{iS}(t_i')\cdot \left(v_i'(t_i', S)-v_i(t_i, S)\right)+\epsilon$.
	\end{enumerate}
	$\rev(M, v, D)$ is the revenue of the mechanism $M$ while the buyers' types are drawn from $D$ and their valuations are $v$ (similarly defined for $\rev(M', v', D')$). $\sigma'_{iS}(t_i')$ is the probability of buyer $i$ receiving exactly bundle $S$ when her reported type is $t_i'$ in mechanism $M'$ with respect to $D'$ and  $\sigma_{iS}(t_i)$ is the probability for the same event in mechanism $M$ with respect to $D$.%$M^{(\beta)}_i(t)$ is the allocation for buyer $i$ in $M^{(\beta)}$ when the reported profile is $t$. \yangnote{Rewrite using $\sigma$}
\end{lemma}

\begin{prevproof}{lemma}{lem:relaxed valuation stronger}
Readers who are familiar with the $\epsilon$-BIC to BIC reduction~\cite{HartlineKM11, BeiH11,DaskalakisW12} might have already realized that the problem here is quite similar. Our proof will follow essentially the same approach.

First, we construct mechanism $M'$, which has two phases:
\vspace{.1in}

\noindent{\bf Phase 1: Surrogate Sale}
\begin{enumerate}
	\item For each buyer $i$, create $\ell-1$ \emph{replicas} sampled i.i.d. from $D_i'$ and $\ell$ \emph{surrogates} sampled i.i.d. from $D_i$. The value of $\ell$ will be specified later.
	\item Ask each buyer to report her type $t_i'$.
	\item For each buyer $i$, create a weighted bipartite graph with the replicas and the bidder $i$ on the left and the surrogates on the right. The edge weight between a replica (bidder $i$) with type $r_i$ and a surrogate with type $s_i$ is the expected value for a bidder with valuation $v_i'(r_i,\cdot)$ to receive bidder $i$'s interim allocation in $M$ when she reported $s_i$ as her type subtract the expected payment of bidder $i$ multiplied by $(1-\eta)$. Formally, the weight is $\sum_{S} \sigma_{iS}(s_i)\cdot v_i'(r_i,S) - (1-\eta)p_i(s_i).$
	\item Compute the VCG matching and prices on the bipartite graph created for each buyer $i$. If a replica (or bidder $i$) is unmatched in the VCG matching, match her to a random unmatched surrogate. The surrogate selected for buyer $i$ is whoever she is matched to.
\end{enumerate}

\vspace{.1in}
\noindent{\bf Phase 2: Surrogate Competition}
\begin{enumerate}
	\item Apply mechanism $M$ on the type profiles of the selected surrogates $\vec{s}$. Let $M_i(\vec{s})$ and $P_i(\vec{s})$ be the corresponding allocated bundle and payment of buyer $i$.
	\item If buyer $i$ is matched to her surrogate in the VCG matching, give her bundle $M_i(\vec{s})$ and charge her $(1-\eta)\cdot P_i(\vec{s})$ plus the VCG price. If buyer $i$ is not matched in the VCG matching, award them nothing and charge them nothing.
	\end{enumerate}

\begin{lemma}[\cite{HartlineKM11}]\label{lem:same distribution}
	If all buyers play $M'$ truthfully, then the distribution of types of the surrogate chosen for buyer $i$ is exactly $D_i$.
\end{lemma}
\begin{proof}
In the mechanism, first the buyer $i$'s type and $\ell-1$ replicas are sampled i.i.d. from the distribution $D_i'$, while $\ell$ surrogates are sampled i.i.d. from the distribution $D_i$. Now, imagine a different order of sampling. We first sample the $\ell$ replicas and $\ell$ surrogates, then we pick one replica to be buyer $i$ uniformly at random. The two different orders above provide exactly the same joint distribution over the replicas, surrogates and buyer $i$. So we only need to argue that in the second order of sampling, the distribution of types of the surrogate chosen by buyer $i$ is exactly $D_i$. Note that the perfect matching (VCG matching plus the uniform random matching with the leftover replicas/surrogates) only depends on the types but not the identity of the node (replica or buyer $i$). So we can decide who is buyer $i$ after we have decided the perfect matching. Since buyer $i$ is chosen uniformly at random among the replicas, the chosen surrogate is also uniformly at random. Clearly, the distribution of the types of a surrogate chosen uniformly at random is also $D_i$. The assumption that buyer $i$ is reporting truthfully is crucial, because otherwise the distribution of buyer $i$'s reported type will be different from the type of a replica, and in that case, we cannot use the second sampling order.
\end{proof}

\begin{lemma}
	$M'$ is a BIC mechanism with respect to valuation $v'$.
\end{lemma}
\begin{proof}
	We need to argue that for every buyer $i$ reporting truthfully is a best response, if every other buyer is truthful. In the VCG mechanism, buyer $i$ faces a competition with the replicas to win a surrogate.  If buyer $i$ has type $t_i'$, then her value for winning a surrogate with type $s_i$ in the VCG mechanism is  $\sum_{S} \sigma_{iS}(s_i)\cdot v_i'(t_i',S) - (1-\eta)p_i(s_i)$ due to Lemma~\ref{lem:same distribution}. Clearly, if buyer $i$ reports truthfully, the weights on the edges between her and all the surrogates will be exactly her value for winning those surrogates. Since buyer $i$ is in a VCG mechanism, reporting the true edge weights is a dominant strategy for her, therefore reporting truthfully is also a best response for her assuming the other buyers are truthful.
	\end{proof}
	
\begin{lemma}
	For any $i$ and $j$, $\sum_{t_i'\in T_i'}f_i'(t_i')\cdot\sum_{S: j\in S} \sigma'_{iS}(t_i')\leq \sum_{t_i\in T_i}f_i(t_i)\cdot\sum_{S: j\in S}\sigma_{iS}(t_i)$.
\end{lemma}

\begin{proof}
	The LHS is the ex-ante probability for buyer $i$ to win item $j$ in $M'$, and the RHS is the corresponding probability in $M$. By Lemma~\ref{lem:same distribution}, we know the surrogate selected by buyer $i$ is participating in $M$ against all other surrogates whose types are drawn from $D_{-i}$. Therefore, the ex-ante probability for the surrogate chosen by buyer $i$ to win item $j$ is the same as RHS. Clearly, this surrogate's ex-ante probability for winning any item should be at least as large as the ex-ante probability for $i$ to win the item in $M'$.
	\end{proof}
	
Next, we want to compare $\rev(M',v', D')$ with $\rev(M,v, D)$. The following simple Lemma relates both quantities to the expected prices charged to the surrogates by mechanism $M$. As in the proof of Lemma~\ref{lem:same distribution}, we change the order of the sampling. We first sample $\ell$ replicas and $\ell$ surrogates then select a replica uniformly at random to be buyer $i$.
Let $s_i^{k}\in T_i$ and $r_i^{k}\in T_i'$ be the type of the $k$-th surrogate and replica, $\Bs= (s_i^{1},\ldots, s_i^{\ell})$, $\Br=(r_i^{1},\ldots, r_i^{\ell})$ and $V(\Bs,\Br)$ be the VCG matching between surrogates and replicas with types $\Bs$ and $\Br$. 	
\begin{lemma}\label{lem:revenue by surrogates}
For every buyer $i$, her expected payments in $M'$ is at least $$(1-\eta)\cdot\E_{\Bs,\Br}\left[\sum_{s_i^k\in V(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right],$$ and her expected payments in $M$ is $$\E_{\Bs}\left[\sum_{k\in[\ell]} \frac{ p_i(s_i^k)}{\ell}\right].$$
\end{lemma}
\begin{proof}
	The revenue of $M'$ contains two parts -- the prices paid by the chosen surrogates and the revenue of the VCG mechanism. Let's compute the first part. For buyer $i$ and each realization of $\Br$ and $\Bs$ only when the buyer $i$'s chosen surrogate is in $ V(\Bs,\Br)$, $i$ pays the surrogate price. Since each surrogate is selected with probability $1/\ell$, the expected surrogate price paid by buyer $i$ is exactly $(1-\eta)\cdot\E_{\Bs,\Br}\left[\sum_{s_i^k\in V(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right]$. Since the VCG payments are nonnegative, we have proved our first statement.
	
	The expected payment from buyer $i$ in $M$ is $\E_{t_i\sim D_i}\left[p_i(t_i)\right]$. Since all $s_i^k$ is drawn from $D_i$, this is exactly the same as $\E_{\Bs}\left[\sum_{k\in[\ell]} \frac{ p_i(s_i^k)}{\ell}\right]$.
\end{proof}

If the VCG matching is always perfect, then Lemma~\ref{lem:revenue by surrogates} already shows that the revenue of $M'$ is at least $(1-\eta)$ fraction of the revenue of $M$. But since the VCG matching may not be perfect, we need to show that the total expected price from surrogates who are not in the VCG matching is small. We prove this in two steps. First, we consider a different type of matching $X(\Bs,\Br)$ -- a maximal matching that only matches replicas and surrogates that have the same type, and show that the expected cardinality of $X(\Bs,\Br)$ is close to $\ell$. Then we argue that for any realization $\Br$ and $\Bs$ the total payments from surrogates that are in $X(\Bs, \Br)$ but not in $V(\Bs,\Br)$ is small.

\begin{lemma}[\cite{HartlineKM11}]\label{lem:equal type matching}
For every buyer $i$, the expected cardinality of a maximal matching that only matches replicas and surrogates with the same type is at least $\ell-\sqrt{|T_i|\cdot \ell}$.
\end{lemma}


The proof can be found in Hartline et. al.~\cite{HartlineKM11}.
\begin{corollary}\label{cor:bound revenue by X}
Let $\mathcal{R} = \max_{i,t_i\in T_i}\max_{S\in[m]} v_i(t_i,S)$, then
$$\E_{\Bs,\Br}\left[\sum_{s_i^k\in X(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right]\geq \E_{\Bs}\left[\sum_{k\in[\ell]} \frac{ p_i(s_i^k)}{\ell}\right]- \sqrt{\frac{|T_i|}{\ell}}\cdot\mathcal{R}.$$
\end{corollary}
\begin{proof}
	Since $M$ is a IR mechanism when the buyers' valuations are $v$, $\mathcal{R}\geq p_i(t_i)$ for any buyer $i$ and any type $t_i$ of $i$. Our claim follows from Lemma~\ref{lem:equal type matching}.
\end{proof}

Now we implement the second step of our argument. The plan is to show the total prices from surrogates that are unmatched by going from  $X(\Bs,\Br)$ to $V(\Bs,\Br)$. For any $\Bs,\Br$, $V(\Bs,\Br)\cup X(\Bs,\Br)$ can be decompose into a disjoint collection augmenting paths and cycles.  If a surrogate is matched in $X(\Bs,\Br)$ but not in $V(\Bs,\Br)$, then it must be the starting point of an augmenting path. The following Lemma upper bounds the price of this surrogate.
\begin{lemma}\label{lem:bounding the price for each augmenting path}
	For any buyer $i$ and any realization of $\Bs$ and $\Br$, let $P$ be an augmenting path that starts with a surrogate that is in $X(\Bs, \Br)$ but not in $V(\Bs,\Br)$. It has the form of either (a) $\left(s_i^{\rho(1)},r_i^{\theta(1)},s_i^{\rho(2)},r_i^{\theta(2)},\ldots, s_i^{\rho{(k)}}\right)$ when the path ends with a surrogate, or (b)$\left(s_i^{\rho(1)},r_i^{\theta(1)},s_i^{\rho(2)},r_i^{\theta(2)},\ldots, s_i^{\rho{(k)}},r_i^{\theta(k)}\right)$ when the path ends with a replica, where $r_i^{\theta(j)}$ is matched to $s_i^{\rho(j)}$ in $X(\Bs, \Br)$ and matched to $s_i^{\rho(j+1)}$ (whenever $s_i^{\rho(j+1)}$ exists) for any $j$.
	\begin{align*}&\sum_{s_i^{\rho(j)}\in P\cap X(\Bs,\Br)} p_i \left(s_i^{\rho(j)}\right)-\sum_{s_i^{\rho(j)}\in P\cap V(\Bs,\Br)} p_i \left(s_i^{\rho(j)}\right)\leq\\
	 &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\frac{1}{\eta}\cdot\sum_{r_i^{\theta(j)}\in P\cap V(\Bs,\Br)} \sum_S \sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot \left(v_i'(r_i^{\theta(j)},S)-v_i(r_i^{\theta(j)},S)\right).
	\end{align*}
\end{lemma}
\begin{proof}
	Since $r_i^{\theta(j)}$ is matched to $s_i^{\rho(j)}$ in $X(\Bs, \Br)$, $r_i^{\theta(j)}$ must be equal to $s_i^{\rho(j)}$. $M$ is a BIC mechanism when buyers valuations are $v$, therefore the expected utility for reporting the true type is better than lying. Hence, the following holds for all $j$:
	\begin{equation}\label{eq:BIC for M}\sum_S\sigma_{iS}\left(s_i^{\rho(j)}\right)\cdot v_i\left(r_i^{\theta(j)},S\right)-p_i\left(s_i^{\rho(j)}\right)\geq \sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot v_i\left(r_i^{\theta(j)},S\right)-p_i\left(s_i^{\rho(j+1)}\right)	
	\end{equation}

The VCG matching finds the maximum weight matching, so the total edge weights in path $P$ and $V(\Bs,\Br)$ is at least as large as the total edge weights in path $P$ and $X(\Bs,\Br)$. Mathematically, it is the following inequalities.
\begin{itemize}
\item If $P$ has format (a): \begin{align}\label{eq:VCG great a}
&\sum_{j=1}^{k-1} \left(\sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot v_i'\left(r_i^{\theta(j)},S\right)-(1-\eta)\cdot p_i\left(s_i^{\rho(j+1)}\right)\right) \geq	\\
&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\sum_{j=1}^{k-1}\left( \sum_S\sigma_{iS}\left(s_i^{\rho(j)}\right)\cdot v_i'\left(r_i^{\theta(j)},S\right)-(1-\eta)\cdot p_i\left(s_i^{\rho(j)}\right)\right) \nonumber
\end{align}
\item If $P$ has format (b): \begin{align}\label{eq:VCG great b}
&\sum_{j=1}^{k-1} \left(\sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot v_i'\left(r_i^{\theta(j)},S\right)-(1-\eta)\cdot p_i\left(s_i^{\rho(j+1)}\right)\right) \geq	\\
&~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\sum_{j=1}^{k}\left( \sum_S\sigma_{iS}\left(s_i^{\rho(j)}\right)\cdot v_i'\left(r_i^{\theta(j)},S\right)-(1-\eta)\cdot p_i\left(s_i^{\rho(j)}\right)\right) \nonumber
\end{align}

\end{itemize}

Next, we further relax the RHS of inequality~(\ref{eq:VCG great a}) using inequality~(\ref{eq:BIC for M}).
\begin{align*}
	&\text{RHS of inequality~(\ref{eq:VCG great a})}\\
	\geq& \sum_{j=1}^{k-1}\left( \sum_S\sigma_{iS}\left(s_i^{\rho(j)}\right)\cdot v_i\left(r_i^{\theta(j)},S\right)-p_i\left(s_i^{\rho(j)}\right)\right)+ \eta\cdot\sum_{j=1}^{k-1}p_i\left(s_i^{\rho(j)}\right)~~\text{(Lemma~\ref{lem:relaxed larger})}\\
	\geq & \sum_{j=1}^{k-1}\left( \sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot v_i\left(r_i^{\theta(j)},S\right)-p_i\left(s_i^{\rho(j+1)}\right)\right)+ \eta\cdot\sum_{j=1}^{k-1}p_i\left(s_i^{\rho(j)}\right)~~\text{(Inequality~\ref{eq:BIC for M})}\\
\end{align*}
We can obtain the following inequality by combining the relaxation above with the LHS of inequality~(\ref{eq:VCG great a}) and rearrange the terms.
$$\frac{1}{\eta}\cdot\sum_{j=1}^{k-1} \sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot \left(v_i'\left(r_i^{\theta(j)},S\right)-v_i\left(r_i^{\theta(j)},S\right)\right)\geq  p_i\left(s_i^{\rho(1)}\right)-p_i\left(s_i^{\rho(k)}\right).$$
The inequality above is exactly the inequality in the statement of this Lemma when $P$ has format (a).

Similarly, we have the following relaxation when $P$ has format (b):
\begin{align*}
	&\text{RHS of inequality~(\ref{eq:VCG great b})}\\
	\geq& \sum_{j=1}^{k}\left( \sum_S\sigma_{iS}\left(s_i^{\rho(j)}\right)\cdot v_i\left(r_i^{\theta(j)},S\right)-p_i\left(s_i^{\rho(j)}\right)\right)+ \eta\cdot\sum_{j=1}^{k}p_i\left(s_i^{\rho(j)}\right)~~\text{(Lemma~\ref{lem:relaxed larger})}\\
	\geq & \sum_{j=1}^{k-1}\left( \sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot v_i\left(r_i^{\theta(j)},S\right)-p_i\left(s_i^{\rho(j+1)}\right)\right)+ \eta\cdot\sum_{j=1}^{k}p_i\left(s_i^{\rho(j)}\right)~~\text{(Inequality~\ref{eq:BIC for M} and $M$ is IR)}\\
\end{align*}
Again, by combining the relaxation with the LHS of inequality~(\ref{eq:VCG great b}), we can prove our claim when $P$ has format (b).
$$\frac{1}{\eta}\cdot\sum_{j=1}^{k-1} \sum_S\sigma_{iS}\left(s_i^{\rho(j+1)}\right)\cdot \left(v_i'\left(r_i^{\theta(j)},S\right)-v_i\left(r_i^{\theta(j)},S\right)\right)\geq  p_i\left(s_i^{\rho(1)}\right).$$
\end{proof}

\begin{lemma}\label{lem: gap between X and V}
	\begin{align*}
&\E_{\Bs,\Br}\left[\sum_{s_i^k\in X(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right]\leq\\
&~~~~~~~~~~~~~~~\E_{\Bs,\Br}\left[\sum_{s_i^k\in V(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right]+\frac{1}{\eta}\cdot\sum_{t_i\in T_i}\sum_{S\subseteq[m]} f_i(t_i)\cdot\sigma'_{iS}(t_i)\cdot \left(v_i'(t_i, S)-v_i(t_i, S)\right).
	\end{align*}
\end{lemma}
\begin{proof}
	Due to Lemma~\ref{lem:bounding the price for each augmenting path}, for any buyer $i$ and any realization of $\Br$ and $\Bs$,  we have
	$$\sum_{s_i^k\in X(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}-\sum_{s_i^k\in V(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\leq \frac{1}{\eta\cdot\ell}\cdot\sum_{s_i^k \in V(\Bs,\Br)} \sum_S \sigma_{iS}\left(s_i^{k}\right)\cdot \left(v_i'(r_i^{\omega(k)},S)-v_i(r_i^{\omega(k)},S)\right),$$ where $r_i^{\omega(k)}$ is the replica that is matched to $s_i^k$ in $ V(\Bs,\Br)$. If we take expectation over $\Br$ and $\Bs$ on the RHS, the expectation means  whenever mechanism $M'$ awards buyer $i$ (with type $t_i$)  bundle $S$, $\frac{1}{\eta}\cdot\left(v_i'(t_i, S)-v_i(t_i, S)\right)$ is contributed to the expectation. Therefore, the expectation of the RHS is the same as $$\frac{1}{\eta}\cdot\left(
\sum_{t_i\in T_i}\sum_{S\subseteq[m]} f_i(t_i)\cdot\sigma'_{iS}(t_i)\cdot \left(v_i'(t_i, S)-v_i(t_i, S)\right)\right).$$ This completes the proof of the Lemma.
\end{proof}

Now, we are ready to prove Lemma~\ref{lem:relaxed valuation stronger}.
\begin{align*}
	&\rev(M, v, D)\\
	=& \sum_i E_{\Bs}\left[\sum_{k\in[\ell]} \frac{ p_i(s_i^k)}{\ell}\right]~~\text{(Lemma~\ref{lem:revenue by surrogates})}\\
	\leq & \sum_i\left(\E_{\Bs,\Br}\left[\sum_{s_i^k\in X(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right] +\sqrt{\frac{|T_i|}{\ell}}\cdot\mathcal{R}\right)~~\text{(Corollary~\ref{cor:bound revenue by X})}\\
	\leq  &\sum_i \E_{\Bs,\Br}\left[\sum_{s_i^k\in V(\Bs,\Br)} \frac{ p_i(s_i^k)}{\ell}\right]\\
	&~~~~~~~~~~~~+\frac{1}{\eta}\cdot\sum_i \sum_{t_i\in T_i}\sum_{S\subseteq[m]} f_i(t_i)\cdot\sigma'_{iS}(t_i)\cdot \left(v_i'(t_i, S)-v_i(t_i, S)\right)+\sum_i\sqrt{\frac{|T_i|}{\ell}}\cdot\mathcal{R} ~~~\text{(Lemma~\ref{lem: gap between X and V})}\\
	\leq & \frac{1}{1-\eta}\cdot \rev(M',v',D)\\
	&~~~~~~~~~~~~+\frac{1}{\eta}\cdot\sum_i \sum_{t_i\in T_i}\sum_{S\subseteq[m]} f_i(t_i)\cdot\sigma'_{iS}(t_i)\cdot \left(v_i'(t_i, S)-v_i(t_i, S)\right)+\sum_i\sqrt{\frac{|T_i|}{\ell}}\cdot\mathcal{R} ~~~\text{(Lemma~\ref{lem:revenue by surrogates})}
\end{align*}

Since $|T_i|$ and $\cal{R}$ are finite numbers, we can take $\ell$ to be sufficiently large, so that $\sum_i\sqrt{\frac{|T_i|}{\ell}}\cdot\mathcal{R} < \epsilon/(1-\eta)$. Therefore, we finished the proof of Lemma~\ref{lem:relaxed valuation stronger}.
\end{prevproof}







==> spm.tex <==
\section{Sequentially Posted-Price Mechanism with Entry Fee}\label{sec:spm}
Here is the formal specification of the Sequential Posted Price with Entry Fee Mechanism.\\

\begin{algorithm}[ht]
\begin{algorithmic}[1]
\REQUIRE $\xi_{ij}$ is the price for bidder $i$ to purchase item $j$ and $\delta_i(\cdot)$ is bidder $i$'s entry fee function.
\STATE $S\gets [m]$
\FOR{$i \in [n]$}
	\STATE Show bidder $i$ {the} set of available items $S$, and define entry fee as ${\delta_i}(S)$.
    \IF{Bidder $i$ pays the entry fee ${\delta_i}(S)$}
        \STATE $i$ receives her favorite bundle $S_i^{*}$, paying $\sum_{j\in S_i^{*}}\xi_{ij}$.
        \STATE $S\gets S\backslash S_i^{*}$.
    \ELSE
        \STATE $i$ gets nothing and pays $0$.
    \ENDIF
\ENDFOR
\end{algorithmic}
\caption{{\sf Sequential Posted Price with Entry Fee Mechanism}}
\label{alg:seq-mech}
\end{algorithm}

